Measurement of CIB power spectra over large sky areas from Planck HFI maps

We present new measurements of the power spectra of the cosmic infrared background (CIB) anisotropies using the Planck 2015 full-mission HFI data at 353, 545, and 857 GHz over 20000 square degrees. We use techniques similar to those applied for the cosmological analysis of Planck, subtracting dust emission at the power spectrum level. Our analysis gives stable solutions for the CIB power spectra with increasing sky coverage up to about 50% of the sky. These spectra agree well with Hi cleaned spectra from Planck measured on much smaller areas of sky with low Galactic dust emission. At 545 and 857 GHz our CIB spectra agree well with those measured from Herschel data. We find that the CIB spectra at l > 500 are well fitted by a power-law model for the clustered CIB, with a shallow index {\gamma}^cib = 0.53\pm0.02. This is consistent with the CIB results at 217 GHz from the cosmological parameter analysis of Planck. We show that a linear combination of the 545 and 857 GHz Planck maps is dominated by CIB fluctuations at multipoles l > 300.

==> new_Table8.tex <==

$\;$

\begin{table*}
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{\small Goodness-of-fit tests for the individual auto- and cross-frequency spectra, binned with $\Delta \ell = 31$, with respect to the best-fit model (power-law clustered CIB) from the full likelihood analysis for masks 40 and 50. The quantities tabulated are the same as in~\reftab{chi2_binned}. Results are shown for the standard covariance matrix (``original''), which reproduce values from~\reftab{chi2_binned} for convenience, and with the correction for statistically-anisotropic Galactic dust (``dust corrected''). The number of degree of freedom is 74 in all cases. }
\label{t:dresult}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
%\scriptsize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth
   \setbox0=\hbox{\rm 0}
   \digitwidth=\wd0
   \catcode`*=\active
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth
   \setbox0=\hbox{+}
   \signwidth=\wd0
   \catcode`!=\active
   \def!{\kern\signwidth}
%
\halign{\tabskip 0pt#\hfil\tabskip 1.5em&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil\tabskip 0pt\cr                            % Template goes here.
\noalign{\doubleline}
Spectrum& $\chi^2$&$\hat \chi^2$&$\Delta\chi^2/\sqrt{2N_{\rm dof}}$& PTE[\%]& $\chi^2$&$\hat \chi^2$&$\Delta\chi^2/\sqrt{2N_{\rm dof}}$& PTE[\%]\hfil\cr
 %\noalign{\vskip 3pt\hrule\vskip 5pt}
&\multispan4\hfil Mask 40 (original) \hfil&\multispan4\hfil Mask 40 (dust corrected) \hfil\cr
  \noalign{\vskip 3pt\hrule\vskip 5pt}
 $353\times353$&  101.12& $1.37$& 2.23& 1.98& *90.59& $1.22$&1.36& 9.22\cr
 $545\times545$& 126.95& $1.72$& 4.35& 0.01& *90.13& $1.22$&1.33& 9.79\cr 
 $857\times857$& 168.49&$2.28$& 7.76&$<0.1$& 131.32&$1.77$&4.71&$0.1$\cr
 $353\times545$& 100.23& $1.35$& 2.16& 2.29& *91.63& $1.24$&1.45& 8.05\cr 
  $353\times857$& 111.51& $1.51$& 3.08& 0.30& *96.70& $1.31$&1.87& 3.94\cr 
 $545\times857$& 124.94& $1.69$& 4.17& 0.20& 107.52& $1.45$&2.76& 0.66\cr
 \noalign{\vskip 3pt\hrule\vskip 5pt}
&\multispan4\hfil Mask 50 (original) \hfil&\multispan4\hfil Mask 50 (dust corrected) \hfil\cr
  \noalign{\vskip 3pt\hrule\vskip 5pt}
 $353\times353$& *96.44& $1.30$& 1.84& *4.10& *83.06& $1.22$&!0.74& 22.05\cr
 $545\times545$& *92.16& $1.25$& 1.49& *7.50& *70.16& $0.95$&*-0.32& 60.48\cr 
 $857\times857$& 162.86&$2.20$& 7.39&$<0.1$& 107.07&$1.45$&!2.72&*0.72\cr
 $353\times545$& *89.77& $1.21$& 1.30& 10.24& *70.81& $0.96$&*-0.26& 58.36\cr 
  $353\times857$& 105.48& $1.43$& 2.59& *0.95& *80.40& $1.09$&!0.53& 28.56\cr
 $545\times857$& 134.27& $1.81$& 4.95& $<0.1$& *93.40& $1.26$&!1.59& *6.34\cr
        \noalign{\vskip 3pt\hrule\vskip 5pt}
}}
\endPlancktablewide 
\endgroup
\end{table*}




==> table_result.tex <==
\begin{table*}%[ht!]
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Best-fit parameter values and 68\,\% marginalised
  errors from the full likelihood analysis. Results are shown for the power-law CIB model for masks 30,
  40, and 50, and for the halo model template for mask 40 only
  (last column). We also include the results of a joint-mask analysis
  of the power-law model
  that uses spectra for mask 40 and 50. The number of degrees of
  freedom is 14\,687 for the power-law model, 14\,688 for the template
  model, and 29\,390 for the joint-mask analysis.
The frequency correlation coefficients $r^{\rm cib}$ and $r^{\rm ps}$
are omitted here; they are presented in~\reftab{correlation}. We also list the reduced
$\chi^2$ (denoted $\hat \chi^2$) for each fit. }
\label{t:result}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
%\scriptsize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth
   \setbox0=\hbox{\rm 0}
   \digitwidth=\wd0
   \catcode`*=\active
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth
   \setbox0=\hbox{+}
   \signwidth=\wd0
   \catcode`!=\active
   \def!{\kern\signwidth}
%
\halign{\tabskip 0pt#\hfil\tabskip 1.5em&
#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil\tabskip 0pt\cr                            % Template goes here.
\noalign{\doubleline}
Type& Parameter& \multispan5\hfil Best fit $\pm68\,\%$ error\hfil\cr
\omit&\omit& mask 30& mask 40& mask 50& Joint$^{\rm mask 40+50}$& mask
40 (halo model)\cr
 \noalign{\vskip 3pt\hrule\vskip 5pt}
\omit&$\hat \chi^2$ & 1.005 & 0.985& 0.977& 1.024& 0.994\cr
 \noalign{\vskip 3pt\hrule\vskip 5pt}
 CIB& $A_{353}^{\rm cib} (\times10^3)$& $2.50\pm0.07$& *$2.56\pm0.07$&*$2.42\pm0.07$& $2.57\pm0.07$& *$2.63\pm0.06$\cr
 \omit&$A_{545}^{\rm cib} (\times10^5)$& $4.50\pm0.20$& *$4.47\pm0.21$&*$4.25\pm0.21$& $4.69\pm0.18$& *$4.74\pm0.22$\cr 
\omit &$A_{857}^{\rm cib} (\times10^9)$& $1.09\pm0.07$& *$1.09\pm0.07$&*$1.00\pm0.07$& $1.11\pm0.07$& *$1.22\pm0.08$\cr 
\omit& $\gamma^{\rm cib}$& $0.51\pm0.02$& *$0.53\pm0.02$&*$0.54\pm0.03$&
$0.56\pm0.02$& --\cr
 \noalign{\vskip 3pt\hrule\vskip 5pt}
Dust&$A_{353}^{\rm dust} (\times10^3)$&  $4.31\pm0.19$& *$8.76\pm0.22$&$16.44\pm0.29$& *$8.99\pm0.21$, $16.15\pm0.22$& *$8.14\pm0.22$\cr
\omit&$A_{545}^{\rm dust} (\times10^6)$& $1.28\pm0.06$& *$2.61\pm0.11$&*$4.96\pm0.21$& *$2.77\pm0.10$, *$5.00\pm0.18$& *$2.50\pm0.11$\cr 
\omit&$A_{857}^{\rm dust} (\times10^9)$& $6.85\pm0.45$& $15.08\pm0.97$&$28.48\pm1.80$& $15.19\pm0.96$, $27.99\pm1.74$& $14.45\pm0.91$\cr 
 \noalign{\vskip 3pt\hrule\vskip 5pt}
PS&$A_{353}^{\rm ps} (\times10^3)$&  $2.15\pm0.07$& *$2.10\pm0.07$&*$2.25\pm0.07$&$2.10\pm0.06$&*$2.06\pm0.05$\cr
\omit&$A_{545}^{\rm ps} (\times10^5)$& $3.54\pm0.19$& *$3.42\pm0.20$&*$3.64\pm0.20$&$3.50\pm0.18$&*$3.33\pm0.15$\cr 
\omit&$A_{857}^{\rm ps} (\times10^8)$& $7.20\pm0.51$& *$7.34\pm0.53$&*$7.76\pm0.56$&$7.20\pm0.51$&*$6.37\pm0.45$\cr 
 \noalign{\vskip 3pt\hrule\vskip 5pt}
Cal& $cal_{353}$& $1.00\pm0.01$&*$1.00\pm0.01$& *$1.00\pm0.01$& $1.00\pm0.01$& *$1.00\pm0.01$\cr
\omit& $cal_{545}$& $1.05\pm0.04	$& *$1.03\pm0.04$&*$1.04\pm0.04$& $1.07\pm0.04$& *$1.05\pm0.04$\cr
\omit& $cal_{857}$& $1.01\pm0.06$& *$1.01\pm0.06$&*$1.01\pm0.06$& $1.02\pm0.06$& *$1.02\pm0.06$\cr
      \noalign{\vskip 3pt\hrule\vskip 5pt}
}}
\endPlancktablewide 
\endgroup
\end{table*}





\begin{table*}%[ht!]
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Goodness-of-fit tests for the individual auto- and
  cross-frequency spectra, binned with $\Delta \ell=31$. Results are
  shown for mask 40, and in each case are compared to the
  best-fit power-law and halo models for the clustered CIB for the appropriate sky fraction from~\reftab{result}.
  For the joint-mask analysis, the goodness of fit
  of the spectra for mask 40 are shown, but the model is
  the best-fit using both masks. The quantity $\Delta\chi^2 =
  \chi^2-N_{\rm dof}$ is the difference from the expected $\chi^2$,
where the number of degrees of freedom $N_{\rm
    dof} = 74$ in all cases (the number of multipole bins for each spectrum).
The fourth and eighth columns list $\Delta\chi^2$ in units of the expected
dispersion, $\sqrt{2N_{\rm dof}}$, and the fifth and ninth columns list the
probability to exceed (PTE) the tabulated  value of $\chi^2$. 
The spectrum $C_\ell^{\rm clean}$ is a combination of the $857\times
857$, $545\times 857$, and $545\times 545$ spectra designed to remove most of
the Galactic dust emission (see~\refsec{dustclean}).
 }
\label{t:chi2_binned}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
%\scriptsize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth
   \setbox0=\hbox{\rm 0}
   \digitwidth=\wd0
   \catcode`*=\active
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth
   \setbox0=\hbox{$<$}
   \signwidth=\wd0
   \catcode`!=\active
   \def!{\kern\signwidth}
%
\halign{\tabskip 0pt#\hfil\tabskip 1.5em&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil&
\hfil#\hfil\tabskip 0pt\cr                            % Template goes here.
\noalign{\doubleline}
Spectrum& $\chi^2$&$\hat \chi^2$&$\Delta\chi^2/\sqrt{2N_{\rm dof}}$& PTE[\%]& $\chi^2$&$\hat \chi^2$&$\Delta\chi^2/\sqrt{2N_{\rm dof}}$& PTE[\%]\hfil\cr
 %\noalign{\vskip 3pt\hrule\vskip 5pt}
&\multispan4\hfil Power-law\hfil&\multispan4\hfil Power-law (Joint) \hfil\cr
  \noalign{\vskip 3pt\hrule\vskip 5pt}
 $353\times353$&101.12&$1.37$&2.23&!2.0*& *95.02& $1.28$&1.73&!5.0*\cr
 $545\times545$&126.95&$1.72$&4.35&!0.01&102.25&$1.38$&2.32&!1.7*\cr 
 $857\times857$&168.49&$2.28$&7.76&$<$0.01&168.04&$2.27$&7.73&$<$0.01\cr
 $353\times545$&100.23&$1.35$&2.16&!2.3*&*99.40&$1.34$&2.09&!2.6*\cr 
  $353\times857$&111.51&$1.51$&3.08&!0.3*&112.86&$1.53$&3.19& !0.2*\cr 
 $545\times857$&124.94&$1.69$&4.17&!0.02&139.32&$1.88$&5.37& $<$0.01\cr
 $C_\ell^{\rm clean}$&114.47&1.55&3.33&!0.2*&101.73&1.37&2.28&!1.8*\cr
 \noalign{\vskip 3pt\hrule\vskip 5pt}
&\multispan4\hfil halo model template \hfil&\multispan4\hfil halo model template (Joint) \hfil\cr
  \noalign{\vskip 3pt\hrule\vskip 5pt}
  $353\times353$&119.88&1.62&*3.77&!0.06&125.81&1.70&*4.26&!0.02\cr
 $545\times545$&159.35&2.15&*7.02&$<$0.01& 158.18&$2.14$&*6.92&$<$0.01\cr 
 $857\times857$&233.84&3.16&13.14&$<$0.01&202.66&2.74&10.58&$<$0.01\cr
 $353\times545$&157.99&2.14&*6.90&$<$0.01&159.88& $2.16$&*7.06&$<$0.01\cr 
  $353\times857$&135.73&1.83&*5.07&!0.3*&130.38&$1.76$&*4.63&$<$0.01\cr
 $545\times857$&164.05&2.22&*7.40&$<$0.01&157.40&$2.13$&*6.86&$<$0.01\cr
  $C_\ell^{\rm clean}$&389.60&5.26&25.94&$<$0.01&387.07&5.23&25.73&$<$0.01\cr
% \noalign{\vskip 3pt\hrule\vskip 5pt}
%  \multispan6\hfil Mask 40 (halo template) $\hfil\cr
%  \noalign{\vskip 3pt\hrule\vskip 5pt}
%   $353\times353$& 101.95&1.38& $2.30$& 1.74 \cr
% $545\times545$& 138.39&1.87& 5.29& $<0.1$\cr 
% $857\times857$& 191.50&2.59&$9.66$& $<0.1$\cr
% $353\times545$& 138.67&1.87& $5.32$& $<0.1$\cr 
%  $353\times857$& 111.69&1.51& 3.10& 0.31 \cr 
% $545\times857$& 142.70&1.93& 5.65& $<0.1$\cr
        \noalign{\vskip 3pt\hrule\vskip 5pt}
}}
\endPlancktablewide 
\endgroup
\end{table*}

